A Formal Model for Polarization under Confirmation Bias in Social Networks

We describe a model for polarization in multi-agent systems based on Esteban and Ray's standard family of polarization measures from economics. Agents evolve by updating their beliefs (opinions) based on an underlying influence graph, as in the standard DeGroot model for social learning, but under a confirmation bias; i.e., a discounting of opinions of agents with dissimilar views. We show that even under this bias polarization eventually vanishes (converges to zero) if the influence graph is strongly-connected. If the influence graph is a regular symmetric circulation, we determine the unique belief value to which all agents converge. Our more insightful result establishes that, under some natural assumptions, if polarization does not eventually vanish then either there is a disconnected subgroup of agents, or some agent influences others more than she is influenced. We also prove that polarization does not necessarily vanish in weakly-connected graphs under confirmation bias. Furthermore, we show how our model relates to the classic DeGroot model for social learning. We illustrate our model with several simulations of a running example about polarization over vaccines and of other case studies. The theoretical results and simulations will provide insight into the phenomenon of polarization.

==> simulations-specification.tex <==
In this section we specify the mathematical details of the simulations from Section~\ref{sec:simulations}.
Recall that we assume that the set of agents is $\Agents = \{0,1,\ldots,n{-}1\}$,
and we let $i,j$ range over $\Agents$.

\subsection{Initial belief configurations:}%
\label{sec:initial-belief-configurations-specification}
We consider the following initial belief configurations, depicted in Figure~\ref{fig:initial-belief-configurations}:

\begin{itemize}
    \item A \emph{uniform} belief configuration representing a set of agents whose beliefs are as varied as possible, all equally spaced in the interval $[0, 1]$:
    \begin{align*}
        \Bfun{i}{0} = \nicefrac{i}{(n{-}1)}~.
    \end{align*}

    \item A \emph{mildly polarized} belief configuration with agents evenly split into two groups with moderately dissimilar inter-group beliefs compared to intra-group beliefs:
    \begin{align*}
        \Bfun{i}{0} =
        \begin{cases}
            \nicefrac{0.2 i}{\ceil{\nicefrac{n}{2}}} + 0.2, & \text{if $i<\ceil{\nicefrac{n}{2}}$,} \\
            \nicefrac{0.2 (i{-}\ceil{\nicefrac{n}{2}})}{(n{-}\ceil{\nicefrac{n}{2}})} + 0.6 & \text{otherwise.}
        \end{cases}
    \end{align*}

    \item An \emph{extremely polarized} belief configuration
    representing a situation in which half of the
    agents strongly believe the proposition, whereas
    %the other
    half strongly disbelieve it:
    \begin{align*}
        \Bfun{i}{0} =
        \begin{cases}
            \nicefrac{0.2 i}{\ceil{\nicefrac{n}{2}}}, & \text{if $i<\ceil{\nicefrac{n}{2}}$,} \\
            \nicefrac{0.2 (i{-}\ceil{\nicefrac{n}{2}})}{(n{-}\ceil{\nicefrac{n}{2}})} + 0.8, & \text{otherwise.}
        \end{cases}
    \end{align*}

    \item A \emph{tripolar} configuration with
    agents divided into three
    groups:
    \begin{align*}
        \Bfun{i}{0} =
        \begin{cases}
            \nicefrac{0.2 i}{\lfloor\nicefrac{n}{3}\rfloor}, & \text{if $i < \lfloor{\nicefrac{n}{3}}\rfloor$,} \\
            \nicefrac{0.2 (i{-}\lfloor{\nicefrac{n}{3}}\rfloor)}{(\ceil{\nicefrac{2n}{3}}{-}\lfloor{\nicefrac{n}{3}}\rfloor)} + 0.4, & \text{if $\lfloor{\nicefrac{n}{3}}\rfloor \leq i < \ceil{\nicefrac{2n}{3}}$,} \\
            \nicefrac{0.2 (i{-}\ceil{\nicefrac{2n}{3}})}{(n{-}\ceil{\nicefrac{2n}{3}})} + 0.8, & \text{otherwise.}
        \end{cases}
    \end{align*}
\end{itemize}

\subsection{Influence graphs:}%
\label{sec:influence-graphs-specification}
Recalling that we assume that $\Ifun{\agent{i}}{\agent{i}}{=}1$ for every $i{\in}\Agents$, all definitinos below only apply to $i{\neq}j$.
We consider the following influence graphs, depicted in Figure~\ref{fig:interaction-graphs}:

\begin{itemize}
    \item A \emph{$C$-clique} influence graph $\Interclique$,
    in which each agent influences every other with constant
    value $C=0.5$: for all $i{\neq}j$,
    \begin{align*}
        \Ifunclique{\agent{i}}{\agent{j}} = 0.5~.
    \end{align*}
    This represents the particular case of a social network in
    which all agents interact among themselves, and are all immune
    to authority bias.

    \item A \emph{circular} influence graph $\Intercircular$
    representing a social network in which agents can be organized
    in a circle in such a way each agent is only influenced by its
    predecessor and only influences its successor: for all $i{\neq}j$,
    \begin{align*}
        \Ifuncircular{\agent{i}}{\agent{j}} =
        \begin{cases}
            0.5, & \text{if (i{+}1)\,\text{mod}\,n = j,} \\
            0, & \text{otherwise.}
        \end{cases}
    \end{align*}
    This is a simple instance of a balanced graph (in which
    each agent's influence on others is as high as the influence received,
    as in Definition~\ref{def:circulation} ahead), which is a pattern commonly
    encountered in some sub-networks.

    \item A \emph{disconnected} influence graph $\Interdisconnected$
    representing a social network sharply divided into two groups in such a way that agents within the same group
    can considerably influence each other, but not at all
    agents in the other group: for all $i{\neq}j$,
    \begin{align*}
        \Ifundisconnected{\agent{i}}{\agent{j}} =
        \begin{cases}
            0.5, & \text{if $\agent{i},\agent{j}$ are both
     ${<} \ceil{\nicefrac{n}{2}}$ or both ${\geq} \ceil{\nicefrac{n}{2}}$,} \\
            0, & \text{otherwise.}
        \end{cases}
    \end{align*}

    % \todo[inline]{Mário: I added below the specification of the ``faintly communicating'' influence graph, making it compatible with the ``disconnected'' influence graph. Notes that numbers changed since the Festschrift paper, so this new definition needs to be implemented for the new experiments.}
    \item A \emph{faintly communicating} influence graph $\Interfaint$
    representing a social network divided into two groups that
    evolve mostly separately, with only faint communication between them.
    More precisely, agents from within the same group influence each other
    much more strongly than agents from different groups: for all $i{\neq}j$,

    \begin{align*}
        \Ifunfaint{\agent{i}}{\agent{j}} =
        \begin{cases}
            0.5, & \text{if $\agent{i},\agent{j}$ are both
     ${<} \ceil{\nicefrac{n}{2}}$ or both ${\geq} \ceil{\nicefrac{n}{2}}$,} \\
            0.1, & \text{otherwise.}
        \end{cases}
    \end{align*}
    This represents a small, ordinary social network, where some close groups of agents have strong influence on one another, and all agents communicate to some extent.

    \item An \emph{unrelenting influencers} influence graph $\Interunrelenting$
    representing a scenario in which two agents
    (say, $\agent{0}$ and $\agent{n{-}1}$)
    exert significantly stronger influence on every other agent than these other agents have among themselves: for all $i{\neq}j$,

    \begin{align*}
        \Ifununrelenting{\agent{i}}{\agent{j}}=
        \begin{cases}
            0.6, & \text{if $i = 0$ and $j \neq n{-}1$ or $i = n{-}1$
    and $j \neq 0$,} \\
            0, & \text{if $j=0$ or $j=n{-}1$,} \\
            0.1, & \text{if $0\neq i \neq n{-}{1}$ and $0 \neq j \neq n{-}{1}$.}
        \end{cases}
    \end{align*}
    This could represent, e.g., a social network
    in which two totalitarian media companies dominate the news
    market, both with similarly high levels of influence on
    all agents.
    The networks have clear agendas to push forward, and are not influenced in a meaningful way by other agents.

    % \todo[inline]{Mário: I added below the specification of the ``malleable influencers'' influence graph, making it compatible with the ``unrelenting influencers'' influence graph. Notes that numbers changed since the Festschrift paper, so this new definition needs to be implemented for the new experiments.}
    \item A \emph{malleable influencers} influence graph $\Intermalleable$
    representing a social network in which two agents have
    strong influence on every other agent,
    but are barely influenced by anyone else: for all $i{\neq}j$,

    \begin{align*}
        \Ifunmalleable{\agent{i}}{\agent{j}}=
        \begin{cases}
            0.8, & \text{if $i = 0$ and $j \neq n{-}1$,} \\
            0.4, & \text{if $i = n{-}1$ and $j \neq 0$,} \\
            0.1, & \text{if $j=0$ or $j=n{-}1$,} \\
            0.1, & \text{if $0\neq i \neq n{-}{1}$ and $0 \neq j \neq n{-}{1}$.}
        \end{cases}
    \end{align*}
    This scenario could represent a situation similar to the
    \qm{unrelenting influencers} scenario above, with two differences.
    First, one TV network has much higher influence than the other.
    Second, the networks are slightly influenced by all the agents
    (e.g., by checking ratings and choosing what news to cover accordingly).
\end{itemize}

